Enhancing the use of Galactic neutron stars as physical laboratories with precise astrometry

The existence of neutron stars was not confirmed until the discovery of pulsars at radio wavelengths in late 1960s. Since then, these highly compact and magnetized objects have been observed across the electromagnetic spectrum, and widely studied. However, lots of the studies related to neutron stars require precise determination of their distances and proper motions. This thesis focuses on high-precision astrometry of neutron stars using the data from the Very Long Baseline Array (VLBA) and the Gaia space telescope operating, respectively, at radio and optical frequencies. The neutron stars studied in the thesis include the extremely magnetized magnetars, the fast-spinning millisecond pulsars, the gravitational-wave-emitting double neutron stars and neutron star X-ray binaries. As a major accomplishment, this thesis presents the novel analysis and the results of the MSPSRpi project -- the largest astrometric survey of millisecond pulsars, then point out the abundant implications of the astrometric results. Additionally, the release of the astrometric results is bound to facilitate the detection of an ultra-low-frequency gravitational-wave background. Methodologically, this thesis applied advanced VLBI techniques to pulsar astrometry using the original data reduction pipeline psrvlbireduce, which leads to the first two significant magnetar parallaxes, and paves the way for studying magnetar formation channels with their velocity distribution. The astrometry Bayesian inference package sterne, developed during the PhD program, serves as a versatile and powerful tool for the inference of astrometric parameters.

==> Makefile <==
CHAPTERS = chapters/chapter1.tex # chapters/chapter2.tex chapters/chapter3.tex chapters/chapter4.tex chapters/chapter5.tex chapters/chapter6.tex

APPENDICES = appendices/appendixA.tex #appendices/appendixB.tex

ALL_SOURCES = thesis.tex \
              abstract.tex acknowledgements.tex declaration.tex \
              mybibliography.bib \
              $(CHAPTERS) ${APPENDICES}

all: thesis.pdf

pdf: $(ALL_SOURCES)
	pdflatex --draftmode thesis.tex
	bibtex thesis
	pdflatex --draftmode thesis.tex
	pdflatex thesis.tex

ps: $(ALL_SOURCES)
	latex thesis.tex
	bibtex thesis
	latex thesis.tex
	latex thesis.tex
	dvips thesis.dvi -o thesis.ps

FILE := ../cas_thesis_template_$(shell date +%Y-%m-%d).tar.gz
tar:
	tar -zcf $(FILE) *

backup: $(ALL_SOURCES)
	rsync -r -L . /path/to/backup
	touch backup

clean:
	rm -f *.aux thesis.bbl thesis.blg thesis.dvi thesis.pdf \
	      thesis.lof thesis.log thesis.lot thesis.out thesis.ps thesis.toc


==> prefix.tex <==
\Huge \noindent Thesis structure and norms
\normalsize
\\

\section*{Thesis structure}
\label{sec:thesis_structure}

\section*{Thesis norms}
\label{sec:thesis_norms}
\begin{itemize}
    \item As this thesis consists of paper chapters written at different stages of my PhD, the mathematical symbols in the paper chapters are not unified. Hence, each chapter follows its own mathematical symbol system. In other words, no mathematical symbol is inherited from preceding chapters. The same rule applies to abbreviations.
\end{itemize}



%\textit{ quote --- }
